A Study on the Efficiency and Generalization of Light Hybrid Retrievers

Hybrid retrievers can take advantage of both sparse and dense retrievers. Previous hybrid retrievers leverage indexing-heavy dense retrievers. In this work, we study "Is it possible to reduce the indexing memory of hybrid retrievers without sacrificing performance"? Driven by this question, we leverage an indexing-efficient dense retriever (i.e. DrBoost) and introduce a LITE retriever that further reduces the memory of DrBoost. LITE is jointly trained on contrastive learning and knowledge distillation from DrBoost. Then, we integrate BM25, a sparse retriever, with either LITE or DrBoost to form light hybrid retrievers. Our Hybrid-LITE retriever saves 13X memory while maintaining 98.0% performance of the hybrid retriever of BM25 and DPR. In addition, we study the generalization capacity of our light hybrid retrievers on out-of-domain dataset and a set of adversarial attacks datasets. Experiments showcase that light hybrid retrievers achieve better generalization performance than individual sparse and dense retrievers. Nevertheless, our analysis shows that there is a large room to improve the robustness of retrievers, suggesting a new research direction.

==> 03_related_work_long.tex <==
\section{Related Work}
\paragraph{Hybrid Retriever}
integrates the sparse and dense retriever and ranks the documents by interpolating the relevance score from each retriever.
The most popular way to obtain the hybrid ranking is applying linear combination of the sparse/dense retriever scores~\cite{karpukhin2020dense,ma2020zero,luan2021sparse,ma2021simple,luo2022improving}.
Instead of using the scores, \citet{chen2022out} adopts Reciprocal Rank Fusion~\cite{cormack2009reciprocal} to obtain the final ranking by the ranking positions of each candidate retrieved by individual retriever.
\citet{arabzadeh2021predicting} trains a classification model to select one of the retrieval strategies: sparse, dense or hybrid model.
% Besides the hybrid scores, some work also use sparse retrievers' signal to train the dense retriever~\cite{gao2021complement,chen2021salient}. 
Most of the hybrid models rely on heavy dense retrievers, and one exception is \cite{ma2021simple}, where they use linear projection, PCA, and product quantization~\cite{jegou2010product} to compress the dense retriever component. 
Our hybrid retrievers use DrBoost as the dense retriever, which is more memory-efficient and achieves better performance than the methods used in \cite{ma2021simple}. More importantly, we introduce a LITE dense retriever to further reduce the indexing memory. 
% Our hybrid models rank the document using linear summation of each retriever (without learning the weights of each component as we find that learning the weights using development set do not generalize well).
% Our contribution is to assess if a light dense retriever is enough to complement the sparse retriever. 

\paragraph{Indexing-Efficient Dense Retriever}
% Here, we discuss the indexing for dense retrievers. 
Most of the existing dense retrievers are indexing heavy~\cite{karpukhin2020dense,khattab2020colbert,lee2021learning,luo2022neural}.
To improve the indexing efficiency, there are mainly three types of techniques. 
One is to use vector product quantization~\cite{jegou2010product}.  
Second is to compress a high dimension dense vector to a low dimension dense vector, for e.g. from 768 to 32 dimension~\cite{lewis2021boosted,ma2021simple}.  
% DrBoost~\cite{lewis2021boosted} is one such work. 
The third  way is to use a binary vector. 
BPR~\cite{yamada2021efficient} and JPQ~\cite{zhan2021jointly} produce the document indexing by 768 dimension binary vectors.

\paragraph{Generalization of IR}
Two main benchmarks have been proposed to study the OOD generalization of retrievers, BEIR~\cite{thakur2021beir} and EntityQuestion~\cite{sciavolino2021simple}.
As shown by previous work~\cite{thakur2021beir,chen2022out}, the generalization is one major concern of DR. 
To address this limitation, \citet{wang2021gpl} proposed GPL, a domain adaptation technique to generate synthetic question-answer pairs in specific domains. 
A follow-up work~\citet{thakur2022domain} trains BPR and JPQ  on the GPL synthetic data to achieve efficiency and generalization. 
~\citet{chen2022out} investigates a hybrid model in the OOD setting, yet different from us, they use a heavy DR and do not concern the indexing memory. 
Most existing work studies OOD generalization, and much less attention paid toward the robustness of retrievers~\cite{penha2022evaluating,zhuang2022characterbert,chentowards}. 
To study robustness, \citet{penha2022evaluating} identifies four ways to change the syntax of the queries but not the semantics. 
Our work is a complementary to \citet{penha2022evaluating}, where we leverage adversarial attack techniques~\cite{morris2020textattack} to create six different testing sets for NQ dataset~\cite{kwiatkowski2019nq}.





% However, this method needs to train the model on specific domain and results in separate model for each specific domain. 
% Therefore, it is difficult to apply this method to real world applications which have thousands of domains. 
% Different from theirs, our light hybrid method without any domain-specific training works for every domain. 


% \paragraph{Knowledge Distillation}



==> 08_discussion.tex <==
% \subsection{Replace BM25 with Lexcical-matching Dense Retriever} 
\section{Discussion and Conclusion}

\paragraph{Replace BM25 with Dense Retriever} While our hybrid retrievers save memory indexing compared to existing hybrid retrievers, 
they requires separate retrieval because 
The sparse and dense retrievers use different indexing methods, which increases the inference complexity of the hybrid models. 
A potential method to overcome this issue is SPAR-like approach where a dense retriever model is used to mimic the BM25 behavior so that the hybrid model can be the concatenation of two dense retrievers. 
Such a model is termed as Lambda model. 
Following ~\cite{luan2021sparse}, we use BM25 to generate the training data and train 6 Lambda models that project vectors of 768 dimension to  32/64/96/128/160/192, respectively. 
However, our Lambda models with lower dimensions can not imitate BM25 well and perform worse than BM25. Replacing BM25 with low capacity Lambda models will degrade the hybrid models performance. 
We leave how to sufficiently distill BM25 knowledge to a low dimension Lambda model as a future work. 
% The results are given in Appendix.
% and the ensemble of Lambda and DrBoost-2 are not as good as the hybrid model of BM25 and DrBoost-2. 
 
% In figure \ref{}, we also show the performance of hybrid Lambda with DrBoost-2.
% Compared with the BM25 + DrBoost-2 hybrid model, we see that the performance of lambda model can not match with BM25 hybrid model again. 
% This shows that compressing the vector of a dense retriever is hard to imitate the BM25 behavior. 
% BM25 uses TF-IDF scores and sparse vectors while DrBoost uses the inner-dot of dense vectors to compute the scores. 
% \input{abl_tables/spar_drboost}

\paragraph{Replace DrBoost with other efficient dense retriever} 
As we mention in the related work, there are other options of efficient DR, for example, BPR, which uses  binary vectors to represent the queries and documents. 
However, BPR itself already involves a re-ranking stage which will make the hybrid-BPR more complex. 
It will be an interesting future work to explore if the hybrid model of BM25 and BPR can achieve reasonable performance without the re-ranking stage in BPR. 





==> abl_tables/kd_diff_teacher.tex <==
% \begin{table}[]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lcccc}
%     \toprule
%     \multirow{2}{*}{Teacher Model} &  \multicolumn{2}{c}{Student} &  \multicolumn{2}{c}{Hybrid Student}\\
%     \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%     & R20 & R100& R20 & R100\\
%     \toprule
%     DrBoost (2*32) & 75.5 & 82.8 & 80.0 & 87.2 \\
%     DrBoost (3*32) & 74.9 & 82.6 &80.3 & 87.0 \\
%     DrBoost (4*32) & 74.9 & 83.0 & 79.7 & 87.0 \\
%     DrBoost (5*32) & 74.6 & 82.9 & 79.3 & 86.9 \\
%     DrBoost (6*32) & 74.6 & 83.6 & 79.6 & 86.9 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Train student models with different DrBoost Teachers.}
%     \label{tab:kd_diff_teacher}
% \end{table}

\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Compress} & \multirow{2}{*}{Student } &  \multicolumn{2}{c}{Student} &  \multicolumn{2}{c}{Hybrid Student}\\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    Layer & Dim & R20 & R100& R20 & R100\\
    \toprule
    LP  & 32 & 74.6 & 83.6 & 79.6 & 86.9 \\
    MLP & 32 & 75.5 & 83.4 & 79.7 & 87.4 \\
    LP & 64 & 77.6 & 84.7 &  80.4 & 87.8\\
    \bottomrule
    \end{tabular}
    }
    \caption{Distill the Knowledge from DrBoost with 6 weak learner to student model.}
    \label{tab:kd_from_stage6}
\end{table}

==> abl_tables/spar_drboost.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    \multirow{2}{*}{Metric} & \multicolumn{6}{c}{Dimension} \\
    \cmidrule(lr){2-7}
    & 32 & 64 & 96 & 128 & 160 & 192 \\
    \toprule
    Lambda & 26.9 & 33.0 & 39.2 & 40.9 & 44.2 & 43.2 \\
    Lambda+DrBoost & 32 & 64 & 96 & 128 & 160 & 192 \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{Lambda models with different representation dimension. For Lambda+DrBoost, we choose the strongest DrBoost, i.e. with 6 weak encoders. BM25:X, BM25+DrBoost: X.}
    \label{tab:spar_drboost}
\end{table}

==> analysis.tex <==
\section{Analysis}

==> tables/beir.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    % \begin{tabular}{lc|c|cc|ccc|cc|cc|c|c|ccc}
    \begin{tabular}{lcccccc}
    \toprule
    
    Method(->)  & BM25 & LITE & DrBoost-2  & Hybrid-L & Hybrid-2  \\ 
    \toprule
    MS MARCO  & 0.260 & 0.329 & 0.341 & 0.363 & \textbf{0.373}  \\ 
    \midrule
    TREC-COVID  &  \textbf{0.632} & 0.446 & 0.474 & 0.579 & 0.603  \\
    NFCorpus   & \textbf{0.322} & 0.208 & 0.211 & 0.305 & 0.310  \\
    \midrule
    NQ & 0.306 & 0.325  & 0.349 & \textbf{0.423} & 0.406 \\ 
    HotpotQA  & \textbf{0.633} & 0.201 & 0.232 & 0.549 & 0.564 \\ 
    FiQA-2018  & 0.236 & 0.142 & 0.148 & 0.241 & \textbf{0.249}  \\ 
    \midrule
    ArguAna  & 0.397 & 0.286 & 0.306 & 0.364  & 0.350 \\ 
    Touché-2020  & \textbf{0.442} & 0.267 & 0.250 & 0.391  & 0.375 \\
    \midrule 
    % CQADupStack & SOTA & BM25 & Drboost$^{2}$ & DrBoost$^{6}$ & Hybrid$^{2}$ & Hybrid$^{6}$ \\ 
    Quora  & \textbf{0.787} & 0.378 & 0.387  & 0.747 & 0.775  \\ 
    \midrule
    DBPedia & 0.318 & 0.243  & 0.236 & \textbf{0.346} & 0.344 \\ 
    \midrule
    SCIDOCS & \textbf{0.149} & 0.070  & 0.075 & 0.133 & 0.135 \\ 
    \midrule
    FEVER & 0.678 & 0.473  & 0.498  & 0.724  & \textbf{0.735} \\ 
    Climate-FEVER  & 0.165 & 0.137 & 0.143 & 0.214 & \textbf{0.220} \\
    SciFact & \textbf{0.707} & 0.307 & 0.330 & 0.648 & 0.651 \\ 
    \midrule
    Average & 0.431 & 0.272 & 0.284 & 0.430 & \textbf{0.435} \\ 
    % \hline
    % Avg. & BM25 & LITE & DrBoost-2  & Hybrid-2 & Hybrid-L \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Performance of light retrievers on BEIR in terms of nDCG@10. MS MARCO is evaluated on the Dev set. Hybrid-2: Hybrid-DrBoost-2, Hybrid-L: Hybrid-LITE.}
    \label{tab:beir}
\end{table}



==> tables/gen_entity.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{Method} & Dim & \multicolumn{2}{c}{EntityQuestion}\\
     \cmidrule(lr){3-4}
    & & R20 & R100\\
    \toprule
    {\bf Existing Method} & ~ & ~ \\ 
    \hline
    BM25~\cite{chen2021salient} & - & 71.2 & 79.7 \\
    DPR~\cite{chen2021salient}  & 768 & 49.7 & 63.4 \\
    DPR~\cite{lewis2021boosted}  & 192 & 47.1 & 60.6 \\
    DrBoost~\cite{lewis2021boosted} & 160 & 51.2 & 63.4 \\
    \hline
    {\bf Our Baselines} & ~ & ~ & ~\\
    \hline
    BM25 & - & 72.10 & 80.61 \\
    DrBoost & 64 & 41.31 & 54.16\\
    % DPR & 32 & 30.46 & 44.88 \\
    DrBoost & 160 & 46.00 & 58.06 \\
    \hline
    {\bf Our Light Hybrid} & ~ &~\\
    \hline
    % BM25+DPR & 32 & 70.82 & 80.52 \\
    BM25+DrBoost & 64 & 72.35 & 81.40  \\
    BM25+DrBoost & 160 & 73.87 & 82.11  \\
    % BM25+Lighter & 32 & - & -  \\
    \toprule
    \end{tabular}
    }
    \caption{Performance of existing methods, our baselines and our light hybrid.}
    \label{tab:gen_enity}
\end{table}


==> tables/kd.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Index-M } &  \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{EntityQuestion}\\
     \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    & (GB) & R@20 & R@100 & R@20 & R@100\\
    \toprule
    DrBoost-1 & 2.5 & 70.4 & 80.0 & 31.1 & 45.5 \\
    Student  & 2.5 & 75.1 & 83.4  & 35.0 & 48.1 \\
    Teacher & 5.1 & 77.3 & 84.5 & 41.3 & 54.2 \\
    \hline
    {\bf Hybrid Model } & ~ &~ & ~\\
    \hline
    + DrBoost-1  & 4.9 & 77.7 & 86.2 & 70.8 & 80.5 \\
    + Student    & 4.9 & 79.9 & 87.2 & 71.5 & 80.8 \\
    + Teacher    & 7.5 & 80.4 & 87.5 & 72.4 & 81.4\\
    \toprule
    \end{tabular}
    }
    \caption{Performance of student model with knowledge distillation.}
    \label{tab:kd}
\end{table}


==> tables/two_kd.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    Method & \# QE & \# CE & QE Dim & CE Dim \\
    
    \toprule
    \citet{lewis2021boosted} & 1 & N & N*D & N*D \\ 
    LITE & 1 & 1 & D & D \\ 
    
    \bottomrule
    \end{tabular}
    }
    \caption{Compare knowledge distillation method in \cite{lewis2021boosted} with our method. QE: question encoder, CE: context encoder, N: number of encoders in DrBoost, D: the dimension of each encoder in DrBoost.}
    \label{tab:two_kd}
\end{table}
